GNN-Assisted Phase Space Integration with Application to Atomistics

Overcoming the time scale limitations of atomistics can be achieved by switching from the state-space representation of Molecular Dynamics (MD) to a statistical-mechanics-based representation in phase space, where approximations such as maximum-entropy or Gaussian phase packets (GPP) evolve the atomistic ensemble in a time-coarsened fashion. In practice, this requires the computation of expensive high-dimensional integrals over all of phase space of an atomistic ensemble. This, in turn, is commonly accomplished efficiently by low-order numerical quadrature. We show that numerical quadrature in this context, unfortunately, comes with a set of inherent problems, which corrupt the accuracy of simulations -- especially when dealing with crystal lattices with imperfections. As a remedy, we demonstrate that Graph Neural Networks, trained on Monte-Carlo data, can serve as a replacement for commonly used numerical quadrature rules, overcoming their deficiencies and significantly improving the accuracy. This is showcased by three benchmarks: the thermal expansion of copper, the martensitic phase transition of iron, and the energy of grain boundaries. We illustrate the benefits of the proposed technique over classically used third- and fifth-order Gaussian quadrature, we highlight the impact on time-coarsened atomistic predictions, and we discuss the computational efficiency. The latter is of general importance when performing frequent evaluation of phase space or other high-dimensional integrals, which is why the proposed framework promises applications beyond the scope of atomistics.

==> flowchart.tex <==
\begin{tikzpicture}
\node [data, text width=1.5cm, fill=green!20] at (-5,0) (start) {Initial Geometry};
\node [process, fill=red!20] at (-2,0) (gnn) {\textbf{GNN}};
\node [decision, fill=blue!20] at (2,0) (error) {$L_1<\delta$?};
\node [process, fill=red!20] at (4.75,0) (post) {Post-process};
\node [terminator, text width=1.8cm, fill=green!20] at (7.5,0) (result) {Relaxed $\langle V \rangle, \bar{\bfq}, \Sigma$};
\node [process, text width=1.5cm, fill=red!20] at (-0.5,-1.5) (update) {update $\bar{\bfq},\Sigma$};

\path[connector] (start) -- coordinate[midway](mark1)(gnn);
\path[connector] (gnn) -- coordinate[midway](mark2)(error);
\path[connector] (error) |- coordinate[pos=0.6](mark3)(update);
\path[connector] (update) -| (mark1);
\path[connector] (error) -- coordinate[pos=0.2](mark4)(post);
\path[connector] (post) -- (result);

\node[black, above=0.1 of mark1]{$\bar{\boldsymbol{q}}, \Sigma$};
\node[black, above=0.1 of mark2]{$\langle V \rangle, \langle \boldsymbol{F}\rangle, \langle F^{\text{th}}\rangle$};
\node[black, above=0.1 of mark3]{No};
\node[black, above=0.1 of mark4]{Yes};
\end{tikzpicture}
